An Empirical Study of Speculative Concurrency in Ethereum Smart Contracts

We use historical data to estimate the potential benefit of speculative techniques for executing Ethereum smart contracts in parallel. We replay transaction traces of sampled blocks from the Ethereum blockchain over time, using a simple speculative execution engine. In this engine, miners attempt to execute all transactions in a block in parallel, rolling back those that cause data conflicts. Aborted transactions are then executed sequentially. Validators execute the same schedule as miners. We find that our speculative technique yields estimated speed-ups starting at about 8-fold in 2016, declining to about 2-fold at the end of 2017, where speed-up is measured using either gas costs or instruction counts. We also observe that a small set of contracts are responsible for many data conflicts resulting from speculative concurrent execution.

==> methodology.tex <==
\section{Methodology}
Here we describe the basic structure of our study,
including some paths not taken.

\subsection{Collecting Transaction Data}
We set up an Ethereum node by installing and running the Ethereum's
client implementation in Go, known as \geth.
The \geth client allows one to synchronize with other network nodes 
and reconstruct the blockchain by validating each block.
The client comes packaged with an interface for fetching data
from the blockchain, as well as debugging tools for inspecting
transactions.
The debugging API includes a utility for reproducing the bytecode trace of a given transaction. 

The \geth client can run in various synchronization modes,
which determine what and how much old state the client records.
For example, a client running in \emph{light} mode will keep track
of the blockchain's current state only,
while in \emph{archive} mode,
the client maintains the full log of all previous states. 

The \geth API makes it straightforward to retrieve any given smart
contract's bytecode.
However, the only way to tell how the bytecode affects the blockchain
state is by re-executing each transaction,
We use \geths tracing utility to re-execute transactions.
The client executes in archive mode,
so that it can reference past states.
Unfortunately, reconstructing the blockchain from scratch is much too
slow to be feasible
(an archive blockchain sync on an ordinary computer is too slow to
keep up with the current growth rate),
so as a baseline we obtained a copy of the blockchain from the
ConSenSys archive~\cite{consensys}.
We downloaded a copy of the Ethereum blockchain from its origins in 2016
to early October 2017.
Starting from this base, we used the \geth utilities to synchronize up to December 2017. 

Between these dates,
the Ethereum blockchain contains about $X$ blocks and $Y$ transactions,
way too much data to analyze in detail in a reasonable time with reasonable
resources.
Instead,
we chose seven historical periods between July 2016
(after the DAO debacle) and December 2017.
Each interval spans roughly one week,
with consecutive intervals separated by 11 weeks so that each day of
the month is considered.   
Due to computational limitations,
we analyze every 10th block in each of the seven historical periods.

\subsection{Greedy transaction execution}
Here is how we simulate a historical transaction trace under a
hypothetical concurrent Ethereum virtual machine.
In the EVM's first, \emph{parallel} phase,
the concurrent virtual machine executes transactions \emph{speculatively}.
Each storage location is assigned a lock.
If one transaction attempts to acquire a lock held by another,
the later transaction is rolled back and deferred to the second,
\emph{sequential} phase.
The second phase starts when the parallel phase is complete,
and all deferred transactions are executed in a one-at-a-time order.

\subsubsection{Multiple Phases}
This greedy, two-phase strategy can be generalized to encompass
multiple parallel phases by having
each transaction that was rolled back in one parallel phase
be re-executed in the next parallel phase.
In principle,
multiple parallel phases might provide additional speed-up,
but we found in our experiments that executing two parallel phases
almost always yields less speed-up than executing a single parallel phase,
due to the extra work incurred from rolling back conflicted transactions in the
second parallel phase.
Henceforth, we consider executions with only a single parallel phase.

\subsection{Data Conflicts}
Two transactions \emph{commute} if executing them in parallel yields the same state,
regardless of how they are interleaved.
Transactions that do not commute are said to \emph{conflict}.
At a more granular level,
two bytecode operations \emph{conflict} if applying them in different orders yields
different storage states.

In the EVM,
the \var{SLOAD} and \var{SSTORE} operations read from and write to persistent storage,
and are responsible for nearly every access and modification of the state
By far the most likely conflicts arise from conflicting
\var{SLOAD} and \var{SSTORE} operations.

Other operations that modify state include
the \var{BALANCE} operation,
which reads a given account's balance,
\var{CREATE} and \var{SELFDESTRUCT}, which create and delete contracts.
While conflicts involving these operations are possible,
we neglect them because they are likely to be quite rare.
For example, one transaction might create a new contract,
and another calls the newly created contract in such a way that the
call may or may not arrive before the contract is initialized.

\subsection{Server Architecture}
\todo{explain number of cores}
